False Claims against Model Ownership Resolution

Deep neural network (DNN) models are valuable intellectual property of model owners, constituting a competitive advantage. Therefore, it is crucial to develop techniques to protect against model theft. Model ownership resolution (MOR) is a class of techniques that can deter model theft. A MOR scheme enables an accuser to assert an ownership claim for a suspect model by presenting evidence, such as a watermark or fingerprint, to show that the suspect model was stolen or derived from a source model owned by the accuser. Most of the existing MOR schemes prioritize robustness against malicious suspects, ensuring that the accuser will win if the suspect model is indeed a stolen model. In this paper, we show that common MOR schemes in the literature are vulnerable to a different, equally important but insufficiently explored, robustness concern: a malicious accuser. We show how malicious accusers can successfully make false claims against independent suspect models that were not stolen. Our core idea is that a malicious accuser can deviate (without detection) from the specified MOR process by finding (transferable) adversarial examples that successfully serve as evidence against independent suspect models. To this end, we first generalize the procedures of common MOR schemes and show that, under this generalization, defending against false claims is as challenging as preventing (transferable) adversarial examples. Via systematic empirical evaluation, we show that our false claim attacks always succeed in the MOR schemes that follow our generalization, including in a real-world model: Amazon's Rekognition API.

==> sections/overview.tex <==
\section{System Overview}



==> shepherd-changelog.tex <==

\onecolumn
\bgroup
\def\arraystretch{1.5}

\section*{Changelog}

We thank the reviewers for their detailed and insightful feedback. 
It is very helpful to improve the quality of this paper.
We have endeavored to address all comments. 

In the following table, we list the comments that need to be addressed. 
In the 3rd column (``Response'') we explain how we addressed each comment. The 4th column (``Link'')  is a clickable link  that points to the place in the paper corresponding to the comment/response.
If a review is addressed at multiple locations in the paper, multiple links are provided. 
Each link points to the text that is added (or changed) to address the corresponding comment.
Each link is named by the initial fragment of the text it points to.
%The links are automatically named by their section names, hence, links with the same name may point to different positions within the same section. 
To ease the tracking of changes, we marked the added text in \revision{red}.
%we marked deleted text in red and newly added text in blue.
%For example, \on{this is the old text}{this is the new text}. For the final version we can change the cmd to only display the second text in black. %(see cmd definition).


%\subsection{Major Changes}

% \begin{enumerate}
%     \item We emphasised our basic assumption of the TEE functionalities (See \ref{row:r1_3}).
%     \item We explained how \BFT is resistant to the potential problem of counter-out-of-sync (See \ref{row:r1_4}).
%     \item We changed our claim about the security argument and moved it to appendix (supplemental material): we only provide an informal argument for the correctness of \BFT   (See \ref{row:r1_5}).
%      \item We  added a picture to show the communication structure of \BFT  (See \ref{row:r1_8}).
%       \item We  explained how \BFT switches to normal-case from the fall-back protocol  (See \ref{row:r1_11}).
%       \item We changed our claim about the performance: instead of claiming ``fastest and most scalable BFT'', we claim ``a fast and scalable BFT (See \ref{row:r2_1})''.
%       \item We fixed the misconception between ``separation agreement/execution'' and  ``active/passive state of replicas'' (See \ref{row:r2_5}).
%       \item We did extra experiments (by only having one replica return the full payload and other replicas return the hashes), and updated the results (See \ref{row:r2_13}).
%  \end{enumerate}




% \subsection{Changes According to the Reviews}

\begin{longtable}{p{.065\textwidth} | p{.3\textwidth} | p{.3\textwidth} | p{.2\textwidth}}
Reviewer & Review comment & Response & Link \\\hline



\textlabel{Editor(1)}{row:e_1}

&

Evaluate the attack using the code from Jia et al. that reaches 90\%+ accuracy on CIFAR-10 (and similarly on their CIFAR-100 code) in order to ensure that the attack scales to more accurate models, or provide a convincing argument why this is not possible.

&

We did use the code from Jia et al.
In their code, they use different distributions to initialize $W_0$.
In this version of our paper, we switch to another distribution to initialize $W_0$; now we can get 90.13\% accuracy on CIFAR-10 and 77.03\% accuracy on CIFAR-100.
All of our results are based on these accuracy.


&

\hyperref[e:1:1]{Under this setting, the models achieve...}

~

\fig~\ref{fig:intermediate_model_accuracyl}

\\\hline





\textlabel{Editor(2)}{row:e_2}

&
Evaluate the attack in a setting where the defender uses different hardware than the attacker, or (less preferable) justify why the setting why the adversary knows the verifier's hardware in advance is practical

&

Thanks for your suggestion! We have added experiments following your suggestion.
The results show that the spoof generation time is still smaller than the proof generation time even if $\Adv$ uses a less powerful hardware then $\Prov$.

&

\hyperref[e:2:1]{Next, we show the spoof generation time is smaller than the proof generation time even if...}

~

\fig~\ref{fig:handwares}


\\\hline











\textlabel{Editor(3)}{row:e_3}

&

Verify the soundness of theoretical claims of the attack cost being smaller than the trainer’s cost, especially with respect to the gradient computations taken in the later two attacks.

&

Thanks for your suggestion! We have added the comparisons.

&

\hyperref[e:3:1]{It is easy to see that Attack~II requires...}

~

\hyperref[e:3:2]{Recall that the complexity for Attack~III is...}


\\\hline






\textlabel{Editor(4)}{row:e_4}


&

Empirically verify that the cost of the attack is smaller than training for different random initializations (with the more accurate models)

&

Thanks for your suggestion! We have re-run the experiments with different random initializations.

&

\hyperref[e:4:1]{All experiment were repeated 5 times with different...}

~

\fig~\ref{fig:Attack2_cifar10_eps}~\ref{fig:Attack2_cifar100_eps}~\ref{fig:Attack2_imagenet_eps}~\ref{fig:Attack3_cifar10_eps}~\ref{fig:Attack3_cifar100_eps}~\ref{fig:Attack3_imagenet_eps}~\ref{fig:Attack2_non_overlapping_eps}~\ref{fig:Attack3_non_overlapping_eps}~\ref{fig:handwares}~\ref{fig:intermediate_model_accuracyl}

\\\hline




\textlabel{Editor(5)}{row:e_5}


&
Clarify why the error (Figure 4/5) needs to be defined w.r.t Q

&

Thanks for your suggestion!
We have added a clarification why the error (Figure 4/5) needs to be defined w.r.t $Q$.


&

\hyperref[e:5:1]{Recall that $\Verif$ only verifies
$Q < \frac{S}{k}$ largest updates for each epoch...}




\\\hline\hline






\textlabel{R-A(1)}{row:r1_1}

&
This make intuitive sense: to get a very small gradient, it suffices that the model's loss is close to zero. So one just needs to slightly modify data points so that the model has overly high confidence on them (the attack is essentially building ``unadversarial examples'' here, see Salman et al. 2021)

&

Thanks for pointing this out! We have added Salman et al. to related work.

&

\hyperref[r1:1:1]{Unadversarial examples...}


\\\hline


\textlabel{R-A(2)}{row:r1_2}

&

The third attack applies a heurisitc where $k$ batches of such unadversarial examples are optimized at once. It would be useful to give a bit more intuition for this attack step. 

&
Thanks for your suggestion! We have added an intuition.

&


\hyperref[r1:2:1]{However, since $W_{t-k}, ..., W_{t-1}$ are all very close to each other, ...}

\\\hline


\textlabel{R-A(3)}{row:r1_3}

&
It would be good to show some results with Attack I, even if those are negative. E.g., does Attack I fail because it does not succeed in producing a valid proof, or does it fail because producing the proof is too expensive?

&

Thanks for your suggestion! 
We have added some results with Attack~I.

&

\hyperref[r1:3:1]{Table~\ref{tab:attack~I} shows the evaluation results of Attack~I on CIFAR-10. ...}


\\\hline


\textlabel{R-A(4)}{row:r1_4}

&
The discussion of countermeasures is interesting if somewhat basic. For the model distance countermeasure, you could imagine the following simple extension to your attack: 
...
It seems that the proposed integrity check only works if the verifier knows that the model was trained on a public dataset, which seems somewhat restrictive.

&

Thanks for pointing these out! We have removed these countermeasures.

&

\hyperref[r1:4:1]{\st{Model distance.} ...}

\\\hline\hline


\textlabel{R-B(1)}{row:r2_1}

&

A general suggestion from Knuth is the text should flow if all equations are replaced with "blah", for example by saying the same thing in words even if it's less precise. This is done early on (e.g., II.B does a good job here). But as we get on into III and especially in IV the notation is less fresh in my mind, and there is less help for the reader.

&

Thanks for your suggestion. We have updated our paper by replacing some notations with words.

&


\\\hline

\textlabel{R-B(2)}{row:r2_2}

&


This is especially concerning because Figure 6(a) makes it look like the original model could be trained for nearly 5x fewer steps and still reach nearly identical accuracy. This would make it (almost) always cheaper to train a model from scratch as opposed to using this attack.

~

The paper makes the claim that the attack could be improved by adopting tricks used to train models efficiently, but it's not clear what these tricks are, or if they would work. For the attack to be truly compelling, I would want to see this actually done.

&

Sorry! Figure 6 (it is Figure~\ref{fig:intermediate_model_accuracyl} now) is a bit misleading. 
We have updated it to make it clearer.

~

The ``tricks'' means the state-of-the-art optimizers.
In this version,  we have optimized our attacks with those ``tricks''.
Now, $T'$ is in the same level as $T$, making the countermeasure ``number of training steps'' invalid.


&

\fig~\ref{fig:intermediate_model_accuracyl}

~

\hyperref[r2:2:2]{\st{We further remark that}. ...}

~

\hyperref[r2:2:1]{\st{Number of training steps.} ...}

~

\hyperref[r2:2:3]{The results show that $T'$ can be large enough ...}


\\\hline

\textlabel{R-B(3)}{row:r2_3}

&



It would be good to make the attack work even if the defender uses ``hard'' hyperparameter settings so everything doesn't fit in memory all at once. A memory-hard defense is still hard. It would also be good to add an evaluation to ImageNet as well, in order to really see the ability of this attack to scale.



&

Thanks for your suggestion! 
We have evaluated Attack II on ImageNet with a ``hard'' hyperparameter setting (k=100, Batchsize=128), and it succeeds! 
We also fixed the problem of memory limitation for Attack III, by separately importing the k batches into memory. Then, it succeeds on ImageNet with a ``hard'' hyperparameter setting (k=100,  Batchsize=128).

~

In this version, all of our experiments were conducted in a ``hard'' setting (k=100,  Batchsize=128).
Therefore, the countermeasure ``Checkpointing interval and batch size'' is no longer valid.

&

\hyperref[r2:3:4]{Nevertheless, we still set $k$ as 100 and batch size as 128 for all of our experiments ...}

~

\hyperref[r2:3:5]{\st{Checkpointing interval and batch size.} ...}

~

\hyperref[r2:3:1]{To show that our attacks can scale to ...}

~

\hyperref[r2:3:2]{\fig~\ref{fig:Attack2_imagenet_eps} shows that ...}

~

\hyperref[r2:3:3]{\fig~\ref{fig:Attack3_imagenet_eps} shows that ...}.



\\\hline


\textlabel{R-B(4)}{row:r2_4}

&

Minor comments:

\begin{itemize}
    \item In IV.A there is a number $100^4$,...
    \item In Figure 3 and 4, some of the plots don't have a y axis label that's near the x intercept, making it hard to know where things are. ...
    \item There's some related work that seems entirely unrelated. ...
    \item It's really bold to end the conclusion ``We will also design a PoL mechanism that is both secure and efficient''.
\end{itemize}


&

\begin{itemize}
    \item We have changed the typography.
    \item We have updated those figures.
    \item We have removed those unrelated work.
    \item We have removed that sentence.
\end{itemize}


&




\\\hline\hline


\textlabel{R-C(1)}{row:r3_1}

&

Can you provide a real world example of where the attacker knows the training set but the verifier doesn't? ...


&

We added an example. 


&


\hyperref[r3:1:1]{In~\cite{PoL}, it is assumed that ...}


\\\hline


\textlabel{R-C(2)}{row:r3_2}

&

The defender could try to check if D1 is an adversarial perturbation of D2 (or vice-versa). (Note that this may be a hard problem; but it is not as hard as detecting adversarial examples: in the DoL case, one has access to both datasets, one of which is non-perturbed.) This may introduce a new arms race: the attacker would need to evade both PoL and this second verifier.

&

Thanks for pointing this out!
We have added this discussion to the paper.

&



\hyperref[r3:2:1]{However, $\Verif$ could still check if ...}

\\\hline

\textlabel{R-C(3)}{row:r3_3}

&

If the attacker could evade PoL by starting from a dataset D' that is very different from the original dataset D, then I would be convinced. ...

&

We validated this by running our attacks following your instructions. The results show that our attack can indeed produce the same model given non-overlapping $D$ and $D'$: the results show similar trends with Figure-2 and Figure-4.

&

\hyperref[r3:3:1]{To this end, ...}

~

\fig~\ref{fig:Attack2_non_overlapping_eps} and \fig~\ref{fig:Attack3_non_overlapping_eps}

\\\hline\hline

\textlabel{R-D(1)}{row:r4_1}

&

Phrasing claims less aggressively

&

Thanks for pointing this out!
We have removed all sentences that sound aggressive. 


&

\hyperref[r4:1:1]{\st{Thereby} ...}

~

\hyperref[r4:1:2]{\st{Instead} ...}

~

\hyperref[r4:1:3]{\st{That is to say} ...}

\\\hline

\textlabel{R-D(2)}{row:r4_2}

&

Fix Algorithm 1 \& 2

&

Thanks for pointing this out!
We have fixed Algorithm 1 \& 2.

&

Algorithm~\ref{alg:creation} and Algorithm~\ref{alg:verification}

\\\hline

\textlabel{R-D(3)}{row:r4_3}

&

Sketch a solution to PoL

&

Thanks for your suggestion!
We have added a solution that is based on verifiable computation.

&

\hyperref[r4:3:1]{Verifiable computation (VC) allows a delegator to outsource the execution ...}



\\\hline



\end{longtable}
\egroup
\twocolumn
\newpage
